Hybrid Audio Detection Using Fine-Tuned Audio Spectrogram Transformers: A Dataset-Driven Evaluation of Mixed AI-Human Speech

The rapid advancement of artificial intelligence (AI) has enabled sophisticated audio generation and voice cloning technologies, posing significant security risks for applications reliant on voice authentication. While existing datasets and models primarily focus on distinguishing between human and fully synthetic speech, real-world attacks often involve audio that combines both genuine and cloned segments. To address this gap, we construct a novel hybrid audio dataset incorporating human, AI-generated, cloned, and mixed audio samples. We further propose fine-tuned Audio Spectrogram Transformer (AST)-based models tailored for detecting these complex acoustic patterns. Extensive experiments demonstrate that our approach significantly outperforms existing baselines in mixed-audio detection, achieving 97\% classification accuracy. Our findings highlight the importance of hybrid datasets and tailored models in advancing the robustness of speech-based authentication systems.

==> 7-Acknowledgment.tex <==
\section*{acknowledgment}
This work was partially supported by the the National Science Foundation Grants CCF1909963, CCF2211163, CNS2120396, CNS2304766, CNS2145389, CNS2120276, CCF2000480, CCF2028873, and CNS2120350.
%an ``e'' after the ``g''. Avoid the stilted expression ``one of us (R. B. 
%G.) thanks $\ldots$''. Instead, try ``R. B. G. thanks$\ldots$''. Put sponsor 
%acknowledgments in the unnumbered footnote on the first page.


==> README <==

January 11, 2007


IEEEtran.bst is the official BibTeX style for authors of the Institute of
Electrical and Electronics Engineers (IEEE) Transactions journals and
conferences.

It also may have applications for other academic work such as theses and
technical reports. The alphanumeric and natbib variants extend the
applicability of the IEEEtran bibstyle family to the natural sciences
and beyond.

The IEEEtran bibstyle is a very comprehensive BibTeX style which provides
many features beyond the standard BibTeX styles, including full support
for references of online documents, patents, periodicals and standards.
See the provided user manual for detailed usage information.

The latest version of the IEEEtran BibTeX style can be found at CTAN:

http://www.ctan.org/tex-archive/macros/latex/contrib/IEEEtran/bibtex/

as well as within IEEE's site:

http://www.ieee.org/

Note that the packages at IEEE's site do not contain the natbib and
alphanumeric variants (e.g., IEEEtranN.bst, etc.) as these are not used
for IEEE related work. These files can be obtained on CTAN.

For helpful tips, answers to frequently asked questions and other support,
visit the IEEEtran home page at my website:

http://www.michaelshell.org/tex/ieeetran/


Enjoy!

Michael Shell
http://www.michaelshell.org/

*******
Version 1.12 (2007/01/11) changes:

 1. Fixed bug with unwanted comma before "et al." when an entry contained
    more than two author names. Thanks to Pallav Gupta for reporting this.

 2. Fixed bug with anomalous closing quote in tech reports that have a
    type, but without a number or address. Thanks to Mehrdad Mirreza for
    reporting this.

 3. Use braces in \providecommand in begin.bib to better support
    latex2html. TeX style length assignments OK with recent versions
    of latex2html - 1.71 (2002/2/1) or later is strongly recommended.
    Use of the language field still causes trouble with latex2html.
    Thanks to Federico Beffa for reporting this.

 4. Added IEEEtran.bst ID and version comment string to .bbl output.

 5. Provide a \BIBdecl hook that allows the user to execute commands
    just prior to the first entry.

 6. Use default urlstyle (is using url.sty) of "same" rather than rm to
    better work with a wider variety of bibliography styles.

 7. Changed month abbreviations from Sept., July and June to Sep., Jul.,
    and Jun., respectively, as IEEE now does. Thanks to Moritz Borgmann
    for reporting this.

 8. Control entry types should not be considered when calculating longest
    label width.

 9. Added alias www for electronic/online.

10. Updated full and abbreviated journal name string definitions in
    IEEEfull.bib and IEEEabrv.bib.

11. New IEEEtranSA.bst, IEEEtranN.bst, and IEEEtranSN.bst variants for
    alphanumeric citation tags and natbib compatibility.


********************************** Files **********************************

README                 - This file.

IEEEtran_bst_HOWTO.pdf - The user manual.

IEEEtran.bst           - The standard IEEEtran BibTeX style file. For use
                         with IEEE work.

IEEEtranS.bst          - A version of IEEEtran.bst that sorts the entries.
                         Some IEEE conferences/publications may use/allow
                         sorted bibliographies.

IEEEexample.bib        - An example BibTeX database that contains the
                         references shown in the user manual.

IEEEabrv.bib           - String definitions for the abbreviated names of
                         IEEE journals. (For use with IEEE work.)
                         
IEEEfull.bib           - String definitions for the full names of IEEE
                         journals. (Do not use for IEEE work.)


Carried on CTAN only, for non-IEEE related work:

IEEEtranSA.bst         - Like IEEEtranS.bst, but with alphanumeric citation
                         tags like alpha.bst. Not for normal IEEE use.

EEEtranN.bst          - Like IEEEtran.bst, but based on plainnat.bst and
                         is compatible with Patrick W. Daly's natbib
                         package. Not for normal IEEE use.

IEEEtranSN.bst         - Sorting version of IEEEtranN.bst. Not for normal
                         IEEE use

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran_bst_HOWTO.pdf, IEEEtran.bst, IEEEtranS.bst,
                   IEEEtranSA.bst, IEEEtranN.bst, IEEEtranSN.bst,
                   IEEEexample.bib, IEEEabrv.bib, IEEEfull.bib
                   
***************************************************************************


==> ablation_evaluation.tex <==
\subsection{Ablation Evaluation}

\textbf{Performance with Different Pruning Components.}
To gain insight on the effects of different pruning components on the overall performance, we set the MIXP parameter set $Par=\{0.9, 0.993, 0.3, 0.3, 0.005, 0.85, 1.1, 0.90\}$ and prune the Lenet-5 on the MNIST using the partial pruning components in MIXP (neuron connection pruning and weight pruning ), respectively.

We find that using the connection pruning only can achieve $86\%$ weight CR and $65\%$ FLOPs CR, while using the weight pruning only can achieve $98\%$ weight CR and $89\%$ FLOPs CR. In contrast, the full MIXP can achieve $98\%$ weight CR and $97\%$ FLOPs CR, indicating that both connection and weight pruning play a significant role in improving the performance of MIXP.



\begin{figure}
  \begin{subfigure}[b]{0.16\textwidth}
    \includegraphics[width=\textwidth]{../fig/relation1}
%    \caption{}
    %\label{fig:1}
  \end{subfigure}%
  \begin{subfigure}[b]{0.16\textwidth}
    \includegraphics[width=\textwidth]{../fig/relation2}
%    \caption{}
    %\label{fig:2}
  \end{subfigure}%
   \begin{subfigure}[b]{0.16\textwidth}
    \includegraphics[width=\textwidth]{../fig/relation3}
%    \caption{}
    %\label{fig:3}
  \end{subfigure}
  \caption{Performance with different ${\lambda _c}$, ${\lambda _w}$, ${\beta}$ and ${\theta _{dec}}$}
  \label{fig:ablation}
\end{figure}

{\color{red}

%\textbf{Performance with Different Influence Factor Decrease Rate and Decrease Boundary.}
\textbf{Performance with Different Parameters.}
%To under the impact of the influence factor decrease rate, we test the accuracy drop of our method on Lenet-5 with different decrease rate values(i.e., 0.6, 0.65, 0.7, 0.75, 0.8, 0.85, 0.9, 1).
We also study the impact of hyperparameters by experimenting with Lenet-5 on MNIST using different decrease rates ($\theta_{dec}$) together with different target connection compression rates ($\lambda_c$), weight compression rates ($\lambda_w$), and decrease boundaries ($\beta$).
%As shown in Figure~\ref{fig:ablation}, the accuracy drop decreases to its minimum when influence factor decrease rate increases to 0.9.
Figure~\ref{fig:ablation} shows that when $\theta_{dec}=0.9$, MIXP can generally achieve the minimum accuracy drop. 
Figure~\ref{fig:ablation} (a) and (b) also show that given the minimum accuracy drop, there is a trade-off between $\lambda_c$ and $\lambda_w$ (i.e., $\lambda_c$ cannot exceed $90\%$ when $\lambda_w$ is $90\%$, and $\lambda_w$ cannot exceed $93\%$ when $\lambda_c$ is $90\%$.)

In addition, we observe that when both $\lambda_c$ and $\lambda_w$ are $90\%$,  MIXP achives the best performance when $\beta=0.85$.

{\color{red} 
\textbf{Performance with Different components.}
We conduct the experiments to present the effects of different pruning components on the overall performance. As shown in Table~\ref{table:ablation}, when the pruned model achieves 90\% connection CR only using connection pruning in MIXP, it has 86\% weight CR and 65\% FLOPs reduction. However, under the same achieved connection CR, our full method, MIXP, has 98\% weight CR and 97\% FLOPs reduction. This result demonstrates that adopting weight pruning after the connection pruning could indeed achieve a better compression ratio and lower FLOPs. Moreover, when only using the weight pruning in MIXP, it achieves 89\% FLOPs reduction which is 8\% lower than full MIXP under the same achieved weight CR 98\%. This result shows that the connection pruning could help reduce the FLOPs than using weight pruning alone.
Overall, both connection and weight pruning of our approach play a significant role in improving the performance of MIXP.
}
\begin{table}[!htbp]
	\centering
	\small
	\begin{tabular}
		{m{3.0cm}<{\centering} m{1.4cm}<{\centering} m{1.4cm}<{\centering}  m{1.4cm}<{\centering} }
		\Xhline{2\arrayrulewidth}
		\quad  & Connection CR(\%) & Weight CR(\%)  & FLOPs CR(\%)
		\\ % inserts table %heading		
		\hline
		
		\begin{tabular}{@{}c@{}}MIXP\\(connection pruning only)\end{tabular} &90  & 86 & 65  \\
		\begin{tabular}{@{}c@{}}MIXP\\(weight pruning only)\end{tabular}&-  & 98 & 89 \\
		\begin{tabular}{@{}c@{}}\textbf{MIXP}\end{tabular}&90  &98 & \textbf{97}  \\
		\Xhline{2\arrayrulewidth}
	\end{tabular}
	\caption{Performance with different pruning components in MIXP on Lenet-5.}
	\label{table:ablation}
\end{table}


